Calibrating LLMs with Information-Theoretic Evidential Deep Learning

Fine-tuned large language models (LLMs) often exhibit overconfidence, particularly when trained on small datasets, resulting in poor calibration and inaccurate uncertainty estimates. Evidential Deep Learning (EDL), an uncertainty-aware approach, enables uncertainty estimation in a single forward pass, making it a promising method for calibrating fine-tuned LLMs. However, despite its computational efficiency, EDL is prone to overfitting, as its training objective can result in overly concentrated probability distributions. To mitigate this, we propose regularizing EDL by incorporating an information bottleneck (IB). Our approach IB-EDL suppresses spurious information in the evidence generated by the model and encourages truly predictive information to influence both the predictions and uncertainty estimates. Extensive experiments across various fine-tuned LLMs and tasks demonstrate that IB-EDL outperforms both existing EDL and non-EDL approaches. By improving the trustworthiness of LLMs, IB-EDL facilitates their broader adoption in domains requiring high levels of confidence calibration. Code is available at https://github.com/sandylaker/ib-edl.

==> tables/ablation_ece_bins.tex <==
\begin{table}[t]
    \centering
    \caption{Sensitivity analysis of ECE with respect to the number of bins. We train and test Llama3-8B on the OBQA dataset. The results show that while the ECE values increase slightly as the number of bins increases, the relative rankings of the methods remain consistent.}
    \begin{tabular}{c|cccc}
        \toprule
        Method & Bins = 10 & Bins = 15 & Bins = 25 & Bins = 35 \\
        \midrule
        MAP & \ms{10.45}{0.52} & \ms{10.52}{0.87} & \ms{10.89}{0.67} & \ms{10.99}{1.01} \\
        MCD & \ms{10.31}{0.37} & \ms{10.48}{0.86} & \ms{10.69}{0.59} & \ms{10.83}{0.76} \\
        Ens & \ms{10.11}{0.13} & \ms{10.08}{0.90} & \ms{10.91}{0.40} & \ms{10.92}{0.84} \\
        LA & \ms{5.20}{1.29} & \ms{5.26}{1.30} & \ms{6.33}{1.11} & \ms{6.42}{0.96} \\
        EDL & \ms{8.16}{1.25} & \ms{8.28}{1.62} & \ms{8.78}{1.27} & \ms{9.44}{1.79} \\
        VID & \ms{5.29}{0.50} & \ms{5.99}{1.41} & \ms{7.16}{1.59} & \ms{7.34}{1.17} \\
        I-EDL & \ms{7.31}{0.33} & \ms{7.57}{0.52} & \ms{8.20}{0.46} & \ms{9.01}{0.50} \\
        R-EDL & \ms{4.64}{0.87} & \ms{4.68}{1.35} & \ms{4.81}{1.09} & \ms{5.47}{0.82} \\
        \midrule
        IB-EDL & \ms{2.77}{0.61}[b] & \ms{2.34}{0.61}[b]\ & \ms{3.91}{0.77}[b] & \ms{4.54}{0.52}[b] \\
        \bottomrule
    \end{tabular}
    \label{tab:ablation_ece_bins}
\end{table}


==> tables/full_noisy_llama2_7b.tex <==
\begin{table}[t]
    \centering
    \caption{Fine-tuning Llama2-7B on noisy datasets. In each training dataset, the labels of $30\%$ samples are randomly perturbed. A robust uncertainty-aware method should not only maintain accuracy but also exhibit low calibration error. Non-EDL methods tend to significantly underperform EDL methods in terms of Accuracy. Therefore, the comparison for ECE and NLL is limited to EDL methods, with the best and second-best values among them highlighted.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c| c | c c c c c c}
        \toprule
         Metrics & Method & ARC-C & ARC-E & OBQA & CSQA & SciQ & RACE\\
         \midrule 
         \multirow{9}{*}{Acc $\uparrow$}
            & MAP    & \ms{51.08}{2.96} & \ms{71.39}{2.73} & \ms{73.93}{2.21} & \ms{74.56}{0.31} & \ms{88.63}{0.06} & \ms{76.83}{0.39} \\
            & MCD    & \ms{51.08}{2.96} & \ms{71.40}{2.72} & \ms{73.93}{2.20} & \ms{74.56}{0.32} & \ms{88.64}{0.06} & \ms{76.95}{0.19} \\ 
            & Ens    & \ms{56.10}{3.11} & \ms{76.03}{1.99} & \ms{75.23}{1.06} & \ms{74.59}{0.23} & \ms{88.64}{0.06} & \ms{76.94}{0.22} \\
            & LA     & \ms{53.38}{2.17} & \ms{74.90}{1.76} & \ms{74.57}{2.22} & \ms{74.59}{0.20} & \ms{88.47}{0.21} & \ms{77.04}{0.39} \\
            \cmidrule{2-8}
            & EDL    & \ms{57.16}{3.33} & \ms{76.16}{1.12} & \ms{74.46}{1.33} & \ms{74.65}{0.05} & \ms{89.03}{0.25} & \ms{77.69}{0.44} \\
            & VID    & \ms{57.56}{0.58}[u] & \ms{76.57}{1.79} & \ms{76.67}{1.42} & \ms{75.97}{0.66}[u] & \ms{89.06}{0.21}[u] & \ms{78.75}{0.25}[u] \\
            & I-EDL  & \ms{53.86}{1.25} & \ms{76.08}{0.71} & \ms{77.00}{0.88}[u] & \ms{74.01}{1.28} & \ms{89.26}{0.32}[b] & \ms{76.48}{0.87} \\
            & R-EDL  & \ms{57.00}{0.76} & \ms{76.96}{1.07}[u] & \ms{73.20}{1.44} & \ms{74.36}{0.49} & \ms{87.33}{0.49} & \ms{78.01}{0.53} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{59.06}{2.07}[b] & \ms{80.27}{0.48}[b] & \ms{78.13}{0.99}[b] & \ms{76.35}{0.66}[b] & \ms{89.06}{0.50}[u] & \ms{79.41}{0.59}[b] \\
        \midrule
        \multirow{9}{*}{ECE $\downarrow$}
            & MAP    & \ms{21.89}{0.11} & \ms{8.95}{1.04} & \ms{8.21}{0.78} & \ms{4.45}{1.51} & \ms{19.05}{0.17} & \ms{15.87}{0.30} \\
            & MCD    & \ms{21.87}{0.12} & \ms{8.91}{1.10} & \ms{8.23}{0.82} & \ms{4.47}{1.55} & \ms{19.04}{0.16} & \ms{15.84}{0.26} \\ 
            & Ens    & \ms{8.24}{1.18}  & \ms{7.83}{0.28} & \ms{11.63}{1.12} & \ms{4.42}{1.52} & \ms{18.91}{0.12} & \ms{15.90}{0.94} \\
            & LA     & \ms{7.12}{1.06}  & \ms{27.02}{1.39} & \ms{22.06}{2.11} & \ms{22.57}{0.09} & \ms{26.28}{0.04} & \ms{24.70}{0.24} \\
            \cmidrule{2-8}
            & EDL    & \ms{8.38}{1.91}[b]  & \ms{26.16}{4.44} & \ms{35.64}{2.97} & \ms{44.29}{2.42} & \ms{46.47}{0.24} & \ms{30.59}{1.14} \\
            & VID    & \ms{19.14}{0.99} & \ms{13.28}{1.84}[b] & \ms{15.00}{0.98}[u] & \ms{13.76}{0.90}[u] & \ms{23.49}{0.34}[u] & \ms{21.22}{0.63}[u] \\
            & I-EDL  & \ms{13.97}{9.04} & \ms{35.30}{1.74} & \ms{37.56}{0.53} & \ms{38.77}{1.59} & \ms{48.60}{0.37} & \ms{36.34}{1.09} \\
            & R-EDL  & \ms{12.25}{1.18} & \ms{20.67}{2.30} & \ms{28.02}{2.63} & \ms{33.64}{0.29} & \ms{39.58}{0.56} & \ms{30.42}{0.89} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{11.21}{2.27}[u] & \ms{13.48}{1.61}[u] & \ms{12.30}{1.65}[b] & \ms{10.48}{0.82}[b] & \ms{23.47}{0.31}[b] & \ms{21.15}{0.36}[b] \\
        \midrule
        \multirow{9}{*}{NLL $\downarrow$}
            & MAP    & \ms{1.94}{0.06} & \ms{1.05}{0.09} & \ms{0.74}{0.03} & \ms{0.84}{0.02} & \ms{0.50}{0.01} & \ms{0.73}{0.00} \\
            & MCD    & \ms{1.94}{0.05} & \ms{1.05}{0.09} & \ms{0.74}{0.03} & \ms{0.81}{0.02} & \ms{0.49}{0.01} & \ms{0.72}{0.02} \\ 
            & Ens    & \ms{1.37}{0.21} & \ms{0.73}{0.06} & \ms{0.73}{0.03} & \ms{0.83}{0.01}[u] & \ms{0.49}{0.01} & \ms{0.73}{0.01} \\
            & LA     & \ms{1.32}{0.06} & \ms{1.03}{0.03} & \ms{0.85}{0.00}[u] & \ms{0.92}{0.01} & \ms{0.56}{0.00} & \ms{0.81}{0.00} \\
            \cmidrule{2-8}
            & EDL    & \ms{1.19}{0.03}[u] & \ms{0.97}{0.03} & \ms{1.05}{0.02} & \ms{1.35}{0.11} & \ms{0.92}{0.01} & \ms{0.90}{0.03} \\
            & VID    & \ms{1.27}{0.01} & \ms{0.83}{0.03} & \ms{0.76}{0.03}[u] & \ms{0.85}{0.01} & \ms{0.54}{0.01}[u] & \ms{0.71}{0.01}[b] \\
            & I-EDL  & \ms{1.29}{0.12} & \ms{1.09}{0.02} & \ms{1.03}{0.01} & \ms{1.20}{0.01} & \ms{0.95}{0.00} & \ms{1.02}{0.01} \\
            & R-EDL  & \ms{1.24}{0.01} & \ms{0.92}{0.01} & \ms{0.95}{0.03} & \ms{1.13}{0.01} & \ms{0.83}{0.01} & \ms{0.93}{0.01} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{1.18}{0.03}[b] & \ms{0.74}{0.03}[b] & \ms{0.71}{0.03}[b] & \ms{0.81}{0.01}[b] & \ms{0.52}{0.01}[b] & \ms{0.71}{0.01}[b] \\
         \bottomrule
    \end{tabular}
    }
    \label{tab:full_noisy_llama2_7b}
\end{table}

==> tables/full_noisy_llama3_8b.tex <==
\begin{table}[t]
    \centering
    \caption{Fine-tuning Llama3-8B on noisy datasets. In each training dataset, the labels of $30\%$ samples are randomly perturbed. A robust uncertainty-aware method should not only maintain accuracy but also exhibit low calibration error. Non-EDL methods tend to significantly underperform EDL methods in terms of Accuracy. Therefore, the comparison for ECE and NLL is limited to EDL methods, with the best and second-best values among them highlighted.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c| c | c c c c c c}
        \toprule
         Metrics & Method & ARC-C & ARC-E & OBQA & CSQA & SciQ & RACE\\
         \midrule 
         \multirow{9}{*}{Acc $\uparrow$}
            & MAP    & \ms{57.71}{0.42} & \ms{80.34}{1.47} & \ms{78.78}{1.00} & \ms{77.04}{0.41} & \ms{92.60}{0.53} & \ms{86.93}{0.11} \\
            & MCD    & \ms{57.71}{0.42} & \ms{80.37}{1.46} & \ms{79.00}{0.92} & \ms{77.05}{0.41} & \ms{92.87}{0.12} & \ms{86.93}{0.12} \\ 
            & Ens    & \ms{63.39}{1.09} & \ms{84.63}{0.53} & \ms{80.61}{0.53} & \ms{77.62}{0.41} & \ms{92.97}{0.06} & \ms{86.93}{0.07} \\
            & LA     & \ms{66.62}{1.08} & \ms{82.64}{0.50} & \ms{79.59}{0.72} & \ms{77.80}{0.49} & \ms{92.93}{0.21} & \ms{87.00}{0.01} \\
            \cmidrule{2-8}
            & EDL    & \ms{69.43}{0.98}[b] & \ms{87.57}{0.13} & \ms{85.60}{0.72} & \ms{79.14}{0.41} & \ms{92.90}{0.40} & \ms{86.26}{0.76} \\
            & VID    & \ms{66.58}{1.92} & \ms{87.67}{0.99}[u] & \ms{84.86}{1.01} & \ms{79.66}{1.26}[b] & \ms{93.23}{0.25} & \ms{86.86}{0.26}[u] \\
            & I-EDL  & \ms{63.87}{2.65} & \ms{84.06}{2.80} & \ms{84.26}{0.42} & \ms{78.02}{0.87} & \ms{92.53}{0.37} & \ms{86.01}{0.51} \\
            & R-EDL  & \ms{71.25}{1.20} & \ms{84.91}{3.91} & \ms{85.73}{0.70}[u] & \ms{78.57}{0.21} & \ms{93.56}{0.05}[b] & \ms{86.16}{0.42} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{68.53}{0.25}[u] & \ms{88.05}{0.43}[b] & \ms{86.13}{0.51}[b] & \ms{79.59}{0.79}[u] & \ms{93.46}{0.38}[u] & \ms{87.01}{0.20}[b] \\
        \midrule
        \multirow{9}{*}{ECE $\downarrow$}
            & MAP    & \ms{13.26}{0.85} & \ms{8.52}{0.63} & \ms{3.72}{1.06} & \ms{8.43}{1.04} & \ms{16.29}{0.43} & \ms{19.61}{0.25} \\
            & MCD    & \ms{12.96}{1.15} & \ms{8.51}{0.62} & \ms{4.17}{1.45} & \ms{8.40}{1.07} & \ms{16.29}{0.43} & \ms{19.64}{0.26} \\ 
            & Ens    & \ms{10.41}{0.74} & \ms{11.09}{0.59} & \ms{4.24}{1.91} & \ms{8.21}{0.21} & \ms{16.15}{0.16} & \ms{19.69}{0.23} \\
            & LA     & \ms{19.02}{0.78} & \ms{23.63}{1.74} & \ms{11.61}{0.29} & \ms{18.05}{0.86} & \ms{18.36}{0.37} & \ms{20.99}{0.18} \\
            \cmidrule{2-8}
            & EDL    & \ms{11.01}{0.79} & \ms{24.29}{0.81} & \ms{41.29}{0.62} & \ms{34.19}{1.93} & \ms{48.36}{0.43} & \ms{34.92}{0.46} \\
            & VID    & \ms{5.90}{0.97}[b]  & \ms{19.58}{0.29}[u] & \ms{19.53}{0.77}[u] & \ms{15.22}{1.15}[u] & \ms{26.30}{0.22}[u] & \ms{22.25}{0.25}[b] \\
            & I-EDL  & \ms{9.57}{2.10}  & \ms{33.57}{6.96} & \ms{42.64}{0.36} & \ms{41.89}{1.18} & \ms{50.13}{0.31} & \ms{42.49}{0.20} \\
            & R-EDL  & \ms{14.50}{2.55} & \ms{23.91}{2.93} & \ms{35.09}{0.84} & \ms{30.95}{2.78} & \ms{41.89}{0.15} & \ms{30.74}{0.94} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{6.73}{1.30}[u]  & \ms{19.49}{0.38}[b] & \ms{17.38}{0.52}[b] & \ms{11.73}{1.11}[b] & \ms{25.00}{0.33}[b] & \ms{23.43}{0.32}[u] \\
        \midrule
        \multirow{9}{*}{NLL $\downarrow$}
            & MAP    & \ms{1.39}{0.05}  & \ms{0.78}{0.03}  & \ms{0.64}{0.01}  & \ms{0.83}{0.01}  & \ms{0.39}{0.01} & \ms{0.56}{0.01} \\
            & MCD    & \ms{1.38}{0.02}  & \ms{0.78}{0.03}  & \ms{0.64}{0.03}  & \ms{0.82}{0.02}  & \ms{0.40}{0.01} & \ms{0.57}{0.01} \\ 
            & Ens    & \ms{1.15}{0.05}  & \ms{0.64}{0.03}  & \ms{0.61}{0.01}  & \ms{0.78}{0.02}  & \ms{0.39}{0.01} & \ms{0.57}{0.02} \\
            & LA     & \ms{1.11}{0.01}  & \ms{0.80}{0.02}  & \ms{0.63}{0.02}  & \ms{0.85}{0.01}  & \ms{0.39}{0.00} & \ms{0.57}{0.01} \\
            \cmidrule{2-8}
            & EDL    & \ms{0.94}{0.02}[b]  & \ms{0.70}{0.01}  & \ms{0.92}{0.01}  & \ms{1.04}{0.03}  & \ms{0.85}{0.00} & \ms{0.78}{0.01} \\
            & VID    & \ms{0.98}{0.03}  & \ms{0.62}{0.02}[u]  & \ms{0.63}{0.01}[u]  & \ms{0.80}{0.02}[u]  & \ms{0.49}{0.01}[u] & \ms{0.57}{0.01}[b] \\
            & I-EDL  & \ms{1.03}{0.03}  & \ms{0.87}{0.06}  & \ms{0.96}{0.01}  & \ms{1.16}{0.00}  & \ms{0.89}{0.01} & \ms{0.91}{0.00} \\
            & R-EDL  & \ms{1.00}{0.02}  & \ms{0.76}{0.05}  & \ms{0.83}{0.02}  & \ms{0.99}{0.02}  & \ms{0.72}{0.00} & \ms{0.73}{0.01} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{0.99}{0.02}[u]  & \ms{0.60}{0.01}[b]  & \ms{0.57}{0.01}[b]  & \ms{0.74}{0.02}[b]  & \ms{0.46}{0.01}[b] & \ms{0.57}{0.01}[b] \\
         \bottomrule
    \end{tabular}
    }
    \label{tab:full_noisy_llama3_8b}
\end{table}

==> tables/full_noisy_mistral_7b.tex <==
\begin{table}[t]
    \centering
    \caption{Fine-tuning Mistral-7B on noisy datasets. In each training dataset, the labels of $30\%$ samples are randomly perturbed. A robust uncertainty-aware method should not only maintain accuracy but also exhibit low calibration error. Non-EDL methods tend to significantly underperform EDL methods in terms of Accuracy. Therefore, the comparison for ECE and NLL is limited to EDL methods, with the best and second-best values among them highlighted.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c| c | c c c c c c}
        \toprule
         Metrics & Method & ARC-C & ARC-E & OBQA & CSQA & SciQ & RACE\\
         \midrule 
         \multirow{9}{*}{Acc $\uparrow$}
            & MAP    & \ms{50.65}{0.30} & \ms{66.30}{2.16} & \ms{75.72}{0.46} & \ms{69.81}{0.55} & \ms{92.96}{0.32} & \ms{85.47}{0.35} \\
            & MCD    & \ms{50.65}{0.30} & \ms{66.21}{2.04} & \ms{75.46}{0.24} & \ms{69.77}{0.51} & \ms{92.93}{0.31} & \ms{85.46}{0.35} \\ 
            & Ens    & \ms{58.16}{0.47} & \ms{76.10}{0.86} & \ms{76.93}{2.14} & \ms{74.18}{1.50} & \ms{92.93}{0.39} & \ms{85.62}{0.28} \\
            & LA     & \ms{66.35}{0.63} & \ms{75.48}{1.88} & \ms{78.20}{1.25} & \ms{74.24}{1.01} & \ms{93.02}{0.29} & \ms{85.57}{0.06} \\
            \cmidrule{2-8}
            & EDL    & \ms{61.63}{1.80} & \ms{85.01}{0.23} & \ms{83.20}{1.25}[u] & \ms{76.63}{0.98} & \ms{93.33}{0.06}[u] & \ms{84.91}{0.10} \\
            & VID    & \ms{62.27}{2.18} & \ms{76.98}{1.13} & \ms{82.06}{1.51} & \ms{77.31}{1.01} & \ms{93.20}{0.17} & \ms{85.59}{0.06}[u] \\
            & I-EDL  & \ms{68.28}{1.19}[u] & \ms{79.73}{0.57} & \ms{81.06}{0.81} & \ms{77.41}{0.09}[u] & \ms{93.33}{0.31}[u] & \ms{84.44}{0.28} \\
            & R-EDL  & \ms{76.39}{0.60}[b] & \ms{86.85}{0.69}[b] & \ms{82.76}{1.73} & \ms{77.10}{1.10} & \ms{93.09}{0.78} & \ms{85.07}{0.34} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{66.44}{0.80}[u] & \ms{85.17}{1.39}[u] & \ms{84.33}{0.51}[b] & \ms{77.44}{0.39}[b] & \ms{93.63}{0.21}[b] & \ms{85.68}{0.20}[b] \\
        \midrule
        \multirow{9}{*}{ECE $\downarrow$}
            & MAP    & \ms{18.08}{0.45} & \ms{9.95}{1.18} & \ms{7.83}{0.62} & \ms{9.61}{0.98} & \ms{15.11}{0.28} & \ms{17.80}{0.33} \\
            & MCD    & \ms{18.24}{0.65} & \ms{9.94}{1.18} & \ms{7.82}{0.61} & \ms{9.60}{0.99} & \ms{15.10}{0.27} & \ms{17.80}{0.33} \\ 
            & Ens    & \ms{10.94}{0.21} & \ms{12.40}{0.34} & \ms{7.02}{0.61} & \ms{8.72}{0.29} & \ms{15.09}{0.17} & \ms{18.58}{0.46} \\
            & LA     & \ms{18.50}{1.46} & \ms{17.31}{0.23} & \ms{13.92}{1.45} & \ms{15.04}{0.41} & \ms{18.13}{0.19} & \ms{18.32}{0.59} \\
            \cmidrule{2-8}
            & EDL    & \ms{12.76}{0.41} & \ms{19.84}{0.95} & \ms{32.57}{1.89} & \ms{25.26}{5.63} & \ms{48.55}{0.33} & \ms{34.06}{0.14} \\
            & VID    & \ms{6.27}{0.66}[b]  & \ms{13.17}{0.76}[b] & \ms{13.92}{0.97}[b] & \ms{11.66}{1.17}[u] & \ms{26.45}{0.16}[u] & \ms{22.01}{0.08}[b] \\
            & I-EDL  & \ms{13.14}{1.17} & \ms{21.44}{1.54} & \ms{35.10}{1.07} & \ms{33.29}{1.04} & \ms{50.90}{0.44} & \ms{41.19}{0.27} \\
            & R-EDL  & \ms{17.63}{2.83} & \ms{17.57}{0.42}[u] & \ms{18.55}{1.68} & \ms{21.35}{1.24} & \ms{41.48}{0.26} & \ms{29.40}{0.31} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{7.46}{1.58}[u]  & \ms{19.08}{3.68} & \ms{14.90}{0.50}[u] & \ms{11.58}{0.43}[b] & \ms{25.08}{0.27}[b] & \ms{22.04}{0.06}[u] \\
        \midrule
        \multirow{9}{*}{NLL $\downarrow$}
            & MAP    & \ms{1.67}{0.03}  & \ms{0.98}{0.06}  & \ms{0.73}{0.05}  & \ms{0.98}{0.03}  & \ms{0.38}{0.01} & \ms{0.56}{0.00} \\
            & MCD    & \ms{1.67}{0.03}  & \ms{0.98}{0.06}  & \ms{0.70}{0.03}  & \ms{0.98}{0.03}  & \ms{0.38}{0.01} & \ms{0.56}{0.01} \\ 
            & Ens    & \ms{1.32}{0.01}  & \ms{0.73}{0.03}  & \ms{0.64}{0.04}  & \ms{0.81}{0.02}  & \ms{0.39}{0.01} & \ms{0.57}{0.02} \\
            & LA     & \ms{1.08}{0.03}  & \ms{0.83}{0.03}  & \ms{0.70}{0.03}  & \ms{0.93}{0.01}  & \ms{0.40}{0.01} & \ms{0.56}{0.00} \\
            \cmidrule{2-8}
            & EDL    & \ms{0.93}{0.05}[b]  & \ms{0.67}{0.00}[u]  & \ms{0.82}{0.03}  & \ms{0.99}{0.04}  & \ms{0.85}{0.00} & \ms{0.78}{0.01} \\
            & VID    & \ms{1.04}{0.06}  & \ms{0.74}{0.02}  & \ms{0.63}{0.01}[u]  & \ms{0.84}{0.01}[u]  & \ms{0.50}{0.01}[u] & \ms{0.60}{0.01}[b] \\
            & I-EDL  & \ms{0.96}{0.04}  & \ms{0.76}{0.02}  & \ms{0.90}{0.01}  & \ms{1.05}{0.02}  & \ms{0.89}{0.00} & \ms{0.91}{0.01} \\
            & R-EDL  & \ms{0.93}{0.03}[b]  & \ms{0.64}{0.02}[b]  & \ms{0.64}{0.03}  & \ms{0.97}{0.04}  & \ms{0.72}{0.01} & \ms{0.72}{0.01} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{0.98}{0.02}  & \ms{0.69}{0.03}  & \ms{0.57}{0.01}[b]  & \ms{0.81}{0.01}[b]  & \ms{0.45}{0.01}[b] & \ms{0.60}{0.01}[b] \\
         \bottomrule
    \end{tabular}
    }
    \label{tab:full_noisy_mistral_7b}
\end{table}


==> tables/id_mistral_7b.tex <==
\begin{table}[t]
    \centering
    \caption{Calibration performance of uncertainty-aware methods on fine-tuned Mistral-7B.}
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c| c | c c c c c c}
        \toprule
         Metrics & Method & ARC-C & ARC-E & OBQA & CSQA & SciQ & RACE\\
         \midrule 
         \multirow{9}{*}{Acc $\uparrow$}
            & MAP    & \ms{80.19}{0.68} & \ms{92.07}{0.12} & \ms{88.06}{0.61} & \ms{83.24}{1.47} & \ms{94.73}{0.06}[u] & \ms{86.61}{0.28} \\
            & MCD    & \ms{80.26}{0.52} & \ms{92.13}{0.15} & \ms{88.07}{0.61} & \ms{83.24}{1.47} & \ms{94.73}{0.06}[u] & \ms{86.64}{0.22}[u] \\ 
            & Ens    & \ms{80.48}{0.45} & \ms{92.41}{0.12}[u] & \ms{88.51}{0.18}[u] & \ms{83.41}{1.44}[u] & \ms{94.80}{0.10}[b] & \ms{86.81}{0.21}[b] \\
            & LA     & \ms{78.47}{1.10} & \ms{92.12}{0.11} & \ms{88.19}{0.69} & \ms{83.21}{1.01} & \ms{94.66}{0.16} & \ms{86.34}{0.39} \\
            & EDL    & \ms{80.60}{0.47}[b] & \ms{92.27}{0.44} & \ms{87.23}{1.42} & \ms{83.31}{0.34} & \ms{94.27}{0.23} & \ms{85.70}{0.41} \\
            & VID    & \ms{80.37}{0.39} & \ms{91.85}{0.13} & \ms{88.33}{0.81} & \ms{82.52}{0.54} & \ms{94.17}{0.12} & \ms{86.40}{0.21} \\
            & I-EDL  & \ms{80.46}{1.63} & \ms{92.28}{0.15} & \ms{88.06}{0.31} & \ms{82.91}{0.20} & \ms{94.03}{0.32} & \ms{85.11}{0.61} \\
            & R-EDL  & \ms{80.12}{0.97} & \ms{92.20}{0.15} & \ms{88.33}{0.91} & \ms{83.07}{0.83} & \ms{94.03}{0.31} & \ms{86.07}{0.28} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{80.57}{0.68}[u] & \ms{92.47}{0.12}[b] & \ms{88.73}{0.70}[b] & \ms{83.65}{0.45}[b] & \ms{94.40}{0.26} & \ms{86.40}{0.32} \\
        \midrule
        \multirow{9}{*}{ECE $\downarrow$}
            & MAP    & \ms{19.42}{0.68} & \ms{7.63}{0.16} & \ms{11.29}{0.31} & \ms{15.72}{1.46} & \ms{4.98}{0.06} & \ms{8.43}{0.46} \\
            & MCD    & \ms{19.26}{0.52} & \ms{7.62}{0.16} & \ms{11.22}{0.40} & \ms{15.72}{1.46} & \ms{4.98}{0.06} & \ms{8.42}{0.47} \\ 
            & Ens    & \ms{17.04}{1.58} & \ms{7.03}{0.79} & \ms{8.87}{0.90}  & \ms{14.18}{2.52} & \ms{4.78}{0.13} & \ms{8.21}{0.62} \\
            & LA     & \ms{20.04}{0.62} & \ms{1.57}{0.39}[b] & \ms{4.49}{0.17}[u]  & \ms{15.11}{2.95} & \ms{1.91}{0.46}[b] & \ms{2.94}{0.25}[b] \\
            & EDL    & \ms{6.21}{1.18}  & \ms{6.25}{0.46} & \ms{6.23}{0.56}  & \ms{7.71}{0.86}  & \ms{7.64}{0.85} & \ms{7.75}{0.86} \\
            & VID    & \ms{9.38}{0.46}  & \ms{2.44}{0.16}[u] & \ms{4.88}{0.77}  & \ms{7.32}{0.74}  & \ms{5.62}{0.52} & \ms{4.20}{0.13} \\
            & I-EDL  & \ms{4.70}{2.15}[u]  & \ms{10.94}{1.27} & \ms{9.63}{0.75} & \ms{8.85}{0.44}  & \ms{11.00}{0.30} & \ms{13.16}{0.87} \\
            & R-EDL  & \ms{11.26}{0.18} & \ms{2.86}{1.07} & \ms{5.43}{0.65}  & \ms{6.30}{0.65}[u]  & \ms{4.48}{0.23}[u] & \ms{3.69}{0.52} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{3.60}{1.10}[b]  & \ms{3.49}{1.24}  & \ms{2.27}{0.67}[b]  & \ms{6.02}{0.08}[b]  & \ms{4.99}{1.22} & \ms{3.58}{0.22}[u] \\
        \midrule
        \multirow{9}{*}{NLL $\downarrow$}
            & MAP    & \ms{2.18}{0.14}  & \ms{0.85}{0.03}  & \ms{0.85}{0.02}  & \ms{1.18}{0.06}  & \ms{0.31}{0.01} & \ms{0.52}{0.01} \\
            & MCD    & \ms{2.18}{0.13}  & \ms{0.84}{0.04}  & \ms{0.84}{0.03}  & \ms{1.18}{0.07}  & \ms{0.31}{0.01} & \ms{0.52}{0.02} \\ 
            & Ens    & \ms{1.82}{0.17}  & \ms{0.78}{0.10}  & \ms{0.67}{0.04}  & \ms{1.01}{0.13}  & \ms{0.28}{0.01} & \ms{0.51}{0.03} \\
            & LA     & \ms{0.78}{0.02}  & \ms{0.29}{0.01}[b]  & \ms{0.38}{0.02}[b]  & \ms{0.59}{0.03}[b]  & \ms{0.17}{0.01}[b] & \ms{0.45}{0.03} \\
            & EDL    & \ms{0.71}{0.04}[u]  & \ms{0.35}{0.02}  & \ms{0.47}{0.03}  & \ms{0.63}{0.01}  & \ms{0.27}{0.01} & \ms{0.47}{0.02} \\
            & VID    & \ms{0.76}{0.03}  & \ms{0.36}{0.01}  & \ms{0.46}{0.01}  & \ms{0.68}{0.02}  & \ms{0.24}{0.01} & \ms{0.41}{0.01}[u] \\
            & I-EDL  & \ms{0.71}{0.05}[u]  & \ms{0.38}{0.02}  & \ms{0.45}{0.01}  & \ms{0.65}{0.01}  & \ms{0.29}{0.01} & \ms{0.50}{0.01} \\
            & R-EDL  & \ms{0.77}{0.02}  & \ms{0.33}{0.01}  & \ms{0.41}{0.03}[u]  & \ms{0.64}{0.01}  & \ms{0.24}{0.01} & \ms{0.45}{0.01} \\
            \cmidrule{2-8}
            & IB-EDL & \ms{0.70}{0.01} [b] & \ms{0.32}{0.02}[u]  & \ms{0.41}{0.01}[u]  & \ms{0.61}{0.01}[u]  & \ms{0.23}{0.01}[u] & \ms{0.40}{0.01}[b] \\
         \bottomrule
    \end{tabular}
    }
    \label{tab:id_mistral_7b}
\end{table}


==> tables/ood_calibration_llama3_8b.tex <==
\begin{table}[t]
    \centering
    \caption{Calibration performance of uncertainty-aware methods on fine-tuned Llama3-8B in the OOD setting. The model is trained on OBQA and tested on three different OOD test sets.}
    \resizebox{0.75\textwidth}{!}{
    \begin{tabular}{c| c | c c c}
        \toprule
         Metrics & Method & OBQA $\rightarrow$ ARC-C & OBQA $\rightarrow$ ARC-E & OBQA $\rightarrow$ CSQA \\
         \midrule 
         \multirow{9}{*}{Acc $\uparrow$}
            & MAP & \ms{79.18}{0.45} & \ms{88.06}{0.20} & \ms{69.37}{0.67} \\
            & MCD & \ms{79.16}{0.43} & \ms{88.05}{0.20} & \ms{69.38}{0.68} \\ 
            & Ens & \ms{79.27}{0.25}[u] & \ms{88.15}{0.02}[u] & \ms{69.14}{0.47} \\
            & LA  & \ms{79.38}{0.40}[b] & \ms{88.36}{0.24}[b] & \ms{69.34}{0.58} \\
            & EDL & \ms{78.27}{0.79} & \ms{86.38}{0.87} & \ms{69.34}{0.88} \\
            & VID & \ms{78.27}{0.57} & \ms{87.41}{0.82} & \ms{69.99}{1.07} \\
            & I-EDL & \ms{78.55}{0.30} & \ms{87.55}{0.20} & \ms{70.49}{0.56} \\
            & R-EDL & \ms{78.32}{1.24} & \ms{87.31}{0.93} & \ms{70.62}{1.28}[u] \\
            \cmidrule{2-5}
            & IB-EDL & \ms{78.31}{1.14} & \ms{87.94}{0.22} & \ms{71.29}{0.96}[b] \\
        \midrule
        \multirow{9}{*}{ECE $\downarrow$}
            & MAP & \ms{18.04}{0.38} & \ms{9.63}{0.47} & \ms{27.85}{0.53} \\
            & MCD & \ms{18.06}{0.36} & \ms{9.63}{0.46} & \ms{27.86}{0.46} \\ 
            & Ens & \ms{16.74}{0.13} & \ms{9.19}{0.65} & \ms{27.07}{1.32} \\
            & LA  & \ms{6.61}{0.41} & \ms{3.02}{0.15}[b] & \ms{11.99}{0.72} \\
            & EDL & \ms{7.65}{0.47} & \ms{10.11}{0.85} & \ms{8.32}{1.33} \\
            & VID & \ms{8.74}{1.19} & \ms{3.19}{0.19}[u] & \ms{16.66}{0.73} \\
            & I-EDL & \ms{7.68}{1.19} & \ms{11.38}{0.65} & \ms{5.96}{0.71}[u] \\
            & R-EDL & \ms{5.03}{0.62}[u] & \ms{5.32}{0.46} & \ms{12.84}{1.73} \\
            \cmidrule{2-5}
            & IB-EDL & \ms{4.67}{1.09}[b] & \ms{5.03}{0.15} & \ms{4.51}{0.15}[b] \\
        \midrule
        \multirow{9}{*}{NLL $\downarrow$}
            & MAP & \ms{1.30}{0.02} & \ms{0.71}{0.03} & \ms{2.06}{0.04} \\
            & MCD & \ms{1.33}{0.06} & \ms{0.70}{0.04} & \ms{2.13}{0.13} \\ 
            & Ens & \ms{1.19}{0.03} & \ms{0.68}{0.05} & \ms{2.01}{0.10} \\
            & LA  & \ms{0.73}{0.02} & \ms{0.42}{0.02}[b] & \ms{1.15}{0.01} \\
            & EDL & \ms{0.74}{0.01} & \ms{0.52}{0.01} & \ms{0.98}{0.03} \\
            & VID & \ms{0.78}{0.01} & \ms{0.46}{0.02} & \ms{1.06}{0.02} \\
            & I-EDL & \ms{0.73}{0.02} & \ms{0.53}{0.01} & \ms{0.94}{0.01}[u] \\
            & R-EDL & \ms{0.73}{0.04}[u] & \ms{0.46}{0.01} & \ms{1.00}{0.05} \\
            \cmidrule{2-5}
            & IB-EDL & \ms{0.72}{0.02}[b] & \ms{0.44}{0.02}[u] & \ms{0.93}{0.02}[b] \\
         \bottomrule
    \end{tabular}
    }
    \label{tab:ood_calibration_llama3_8b}
\end{table}


==> tables/ood_mistral_7b.tex <==
\begin{table}[t]
    \centering
    \caption{OOD detection performance on fine-tuned Mistral-7B. $A \rightarrow B$ indicates $A$ as the ID training set and $B$ as the OOD test set. MP and UM are two scores for measuring AUROC.}
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c | c | c c | c c | c c}
        \toprule
        \multirow{3}{*}{Model} & \multirow{3}{*}{Method} & \multicolumn{2}{c|}{OBQA $\rightarrow$ ARC-C} & \multicolumn{2}{c|}{OBQA $\rightarrow$ ARC-E} & \multicolumn{2}{c}{OBQA $\rightarrow$ CSQA} \\
        \cmidrule{3-8} 
         & & \multicolumn{2}{c|}{AUROC $\uparrow$} & \multicolumn{2}{c|}{AUROC $\uparrow$} & \multicolumn{2}{c}{AUROC $\uparrow$} \\
        \cmidrule{3-8}
         & & MP & UM & MP & UM & MP & UM \\
        \midrule
        \multirow{9}{*}{Mistral-7B} & MAP    & \ms{60.40}{1.36} & $-$ & \ms{53.30}{1.16} & $-$ & \ms{63.70}{1.10} & $-$ \\
        & MCD    & \ms{60.39}{1.37} & $-$ & \ms{53.30}{1.16} & $-$ & \ms{63.70}{1.10} & $-$ \\
        & Ens    & \ms{60.67}{0.87} & $-$ & \ms{54.05}{0.88} & $-$ & \ms{63.80}{1.09} & $-$ \\
        & LA     & \ms{61.61}{1.05} & $-$ & \ms{53.14}{0.93} & $-$ & \ms{68.31}{1.11} & $-$ \\
        & EDL    & \ms{84.17}{1.87} & \ms{77.34}{6.97} & \ms{81.81}{2.31} & \ms{74.18}{6.38} & \ms{83.55}{2.67} & \ms{78.28}{5.81} \\
        & VID    & \ms{86.30}{3.85}[u] & \ms{84.74}{0.89}[u] & \ms{88.16}{1.87}[u] & \ms{90.68}{0.17}[u] & \ms{88.93}{1.39}[u] & \ms{81.45}{2.04} \\
        & I-EDL  & \ms{85.02}{0.90} & \ms{82.28}{1.44} & \ms{82.67}{1.34} & \ms{79.42}{2.33} & \ms{85.08}{0.87} & \ms{82.07}{1.43}[u] \\
        & R-EDL  & \ms{76.26}{1.05} & \ms{72.85}{0.61} & \ms{71.95}{0.78} & \ms{67.56}{0.72} & \ms{75.59}{1.32} & \ms{71.93}{2.05} \\
        \cmidrule{2-8}
        & IB-EDL & \ms{90.28}{1.22}[b] & \ms{88.53}{1.08}[b] & \ms{89.54}{1.16}[b] & \ms{94.29}{0.49}[b] & \ms{90.45}{1.13}[b] & \ms{83.85}{2.55}[b] \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:ood_mistral_7b}
\end{table}


==> tables/ood_mmlu_math_llama2_7b.tex <==
\begin{table}[t]
    \centering
    \caption{OOD Detection AUROC on Llama3-8B in the setting OBQA $\rightarrow$ MMLU-Math. IB-EDL achieves the best performance even under significant distribution shifts, such as transitioning from a common-sense reasoning dataset like OBQA to a math-focused OOD dataset.}
    \begin{tabular}{c|cc}
        \toprule
        \multirow{3}{*}{Method} & \multicolumn{2}{c}{OBQA $\rightarrow$ MMLU-Math} \\
        \cmidrule(lr){2-3}
        & \multicolumn{2}{c}{AUROC $\uparrow$} \\
        \cmidrule(lr){2-3}
        & MP & UM \\
        \midrule
        MAP & \ms{91.36}{0.57} & - \\
        MCD & \ms{90.85}{0.33} & - \\
        Ens & \ms{90.68}{0.80} & - \\
        LA & \ms{91.09}{0.41} & - \\
        EDL & \ms{92.78}{0.26} & \ms{92.86}{0.21} \\
        VID & \ms{91.64}{0.79} & \ms{66.61}{4.98} \\
        I-EDL & \ms{91.48}{0.72} & \ms{90.67}{0.88} \\
        R-EDL & \ms{88.44}{2.11} & \ms{88.22}{1.70} \\
        \cmidrule(lr){1-3}
        IB-EDL & \ms{93.63}{0.66}[b] & \ms{93.64}{0.56}[b] \\
        \bottomrule
    \end{tabular}
    \label{tab:ood_mmlu_math_llama2_7b}
\end{table}



==> tables/train_test_consumption.tex <==
\begin{table}[t]
    \centering
    \caption{Comparison of computational efficiency for various methods using Llama3-8B on the OBQA. IB-EDL demonstrates comparable training and inference speeds as well as memory consumption compared to MAP and other EDL methods, confirming its computational efficiency.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|ccc}
        \toprule
        Method & Test Samples/s $\uparrow$ & Training Samples/s $\uparrow$ & Memory (GB) at Training$\downarrow$ \\
        \midrule
        MAP & \ms{69.55}{2.86} & \ms{26.57}{1.96} & \ms{21.21}{0.35} \\
        MCD (10 forwards) & \ms{9.79}{1.21} & - & - \\
        Ens (3 models) & \ms{25.77}{3.54} & - & - \\
        LA & \ms{5.95}{0.49} & - & - \\
        EDL & \ms{68.99}{1.59} & \ms{26.44}{1.11} & \ms{21.23}{0.15} \\
        VID & \ms{69.17}{0.99} & \ms{26.69}{1.37} & \ms{21.29}{0.37} \\
        I-EDL & \ms{68.94}{2.18} & \ms{26.02}{0.71} & \ms{21.33}{0.11} \\
        R-EDL & \ms{68.84}{1.09} & \ms{26.47}{1.09} & \ms{21.27}{0.21} \\
        \midrule
        IB-EDL & \ms{68.08}{1.75} & \ms{26.41}{1.04} & \ms{21.88}{0.66} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:train_test_consumption}
\end{table}

